Keypoint-GraspNet: Keypoint-based 6-DoF Grasp Generation from the Monocular RGB-D input

Great success has been achieved in the 6-DoF grasp learning from the point cloud input, yet the computational cost due to the point set orderlessness remains a concern. Alternatively, we explore the grasp generation from the RGB-D input in this paper. The proposed solution, Keypoint-GraspNet, detects the projection of the gripper keypoints in the image space and then recover the SE(3) poses with a PnP algorithm. A synthetic dataset based on the primitive shape and the grasp family is constructed to examine our idea. Metric-based evaluation reveals that our method outperforms the baselines in terms of the grasp proposal accuracy, diversity, and the time cost. Finally, robot experiments show high success rate, demonstrating the potential of the idea in the real-world applications.

==> figs/figPhyResults.tex <==
\begin{figure*}[t!]
  \vspace*{-0.1in}
  \centering
  \scalebox{0.98}{
    \begin{tikzpicture}
     \node[anchor=north west] at (0in,0in)
      {{\includegraphics[width=1.0\textwidth,clip=true,trim=0in
      9.5in 0.1in 0.035in]{figs/phyResults.pdf}}};
     \node[yshift=-0pt,anchor=north west, fill=white, inner sep=1.4pt] at (0.07in,-0.05in) {\bf \small (a)};
     \node[yshift=-0pt,anchor=north west, fill=white, inner sep=1.4pt] at (1.44in,-0.05in) {\bf \small (b)};
     \node[yshift=-0pt,anchor=north west, fill=white, inner sep=1.4pt] at (2.80in,-0.05in) {\bf \small (c)};
     \node[yshift=-0pt,anchor=north west, fill=white, inner sep=1.4pt] at (4.16in,-0.05in) {\bf \small (d)};
    \end{tikzpicture}
  }
  \vspace*{-0.2in}
  \caption{Physical experiment results.
  (a)(b): Generated grasps for the lying and standing tape object;
  (c)(d): Generated grasps for the cuboid object of the different poses.
  }
 \label{fig:phyResults}
 \vspace*{-0.1in}
\end{figure*}
~                        


==> figs/figVisSingle.tex <==
\begin{figure}[t!]
  \vspace*{-0.0in}
  \centering
  \scalebox{0.98}{
    \begin{tikzpicture}
     \node[anchor=north west] at (0in,0in)
      {{\includegraphics[width=\linewidth,clip=true,trim=0in
      8.0in 3.9in 0.035in]{figs/visResults.pdf}}};
%     \node[yshift=-0pt,anchor=north west] at (0.1in,0.0in) {\bf \small (a)};
%     \node[anchor=north west] at (0.28in, -1.9in) {Training Label};
%     \node[anchor=north west] at (0.9in,-1.9in) {Keypoints \\ Prediction};
    \end{tikzpicture}
  }
  \vspace*{-0.3in}
  \caption{Example results on the synthetic dataset.
  The \netName\ is able to recover the underlying distribution from the training labels (stick and semi-sphere)
  and predict diverse grasp modes (cuboid)
  }
 \label{fig:visResults}
 \vspace*{-0.2in}
\end{figure}


==> probDef.tex <==
%\section{Problem Definition}


==> tables/tabAblKpt.tex <==
\begin{table}[t!]
  \centering
  \setlength\tabcolsep{2.5pt} 
  \renewcommand{\arraystretch}{1.1}
  \begin{threeparttable}
  \begin{tabular}{|c| c | c | c | c | c | c | c | c | c|}
  		\hline
	\multirow{2}{*}{Keypoint + \PnP} &
    \multicolumn{3}{c|}{$1\text{cm}+20^\circ$} &
    \multicolumn{3}{c|}{$2\text{cm}+30^\circ$} & 
    \multicolumn{3}{c|}{$3\text{cm}+45^\circ$}  \\
 		\cline{2-10}
 	{} & GSR & GCR & OSR & GSR & GCR & OSR & GSR & GCR & OSR  \\
 	\hline
 	
 	Box+IPPE	&  \textbf{0.544} & \textbf{0.403} & \textbf{0.946} & \textbf{0.773} & \textbf{0.613} & \textbf{0.989} & \textbf{0.860} & 0.719 & \textbf{0.998}  \\
 	Box+\PnP[3] & 0.511 & 0.391 & 0.938 & 0.759 & 0.611 & 0.985 & 0.858 & \textbf{0.720} & 0.996 \\
 	Box+\EPnP	& 0.058 & 0.070 & 0.542 & 0.114 & 0.180 & 0.680 & 0.166 & 0.309 & 0.757 \\
 	
 		\hline
 		
 	Tail+IPPE	& 0.271 & 0.291 & 0.970 & 0.470 & 0.475 & 0.991 & 0.584 & 0.588 & 0.996 \\
 	Tail+\PnP[3]	& 0.468 & 0.387 & 0.978 & 0.692 & 0.590 & 0.997 & 0.778 & 0.696 & 0.998 \\
 	Tail+\EPnP	& 0.017 & 0.027 & 0.364 & 0.038 & 0.091 & 0.518 & 0.065 & 0.183 & 0.619 \\
 	
 		\hline
 		
 	Tetrahedron+\PnP[3]	 	& 0.339 & 0.314 & 0.886 & 0.573 & 0.521 & 0.917 & 0.690 & 0.640 & 0.925 \\
 	Tetrahedron+\EPnP 	& 0.172 & 0.222 & 0.836 & 0.326 & 0.441 & 0.890 & 0.441 & 0.582 & 0.912 \\
 	
 		\hline
  \end{tabular}
  \caption{Ablation Study on the keypoint type and the \PnP algorithm choices. The box type keypoint achieve the best performance with the IPPE or \PnP[3] algorithm.}
  \label{tab:visAblate}
  \end{threeparttable}
  \vspace*{-0.2in}
\end{table}


==> tables/tabVisMulti.tex <==
\begin{table*}[t!]
  \centering
  \setlength\tabcolsep{2.5 pt} 
  \renewcommand{\arraystretch}{1.1}
  \caption{Multi-object Dataset Evaluation}
  \begin{threeparttable}
  \begin{tabular}{|c| c | c | c | c | c | c | c | c | c | c|}
  		\hline
	\multirow{2}{*}{Methods} &
	\multirow{2}{*}{Train Scene} &
    \multicolumn{3}{c|}{$1\text{cm}+20^\circ$} &
    \multicolumn{3}{c|}{$2\text{cm}+30^\circ$} & 
    \multicolumn{3}{c|}{$3\text{cm}+45^\circ$}  \\ 
 		\cline{3-11}
 	{} & {} & GSR & GCR & OSR & GSR & GCR & OSR & GSR & GCR & OSR  \\
 	\hline
 		
 	PnGPD 				& N/A & 0.	& 0. & 0. & 0.083 & 0.0002 & 0.008 & 0.417 & 0.003 & 0.032  \\
 	6D-GN  	& Single-Obj & 0.002 & 0.001 & 0.007 & 0.02 & 0.005 & 0.053 & 0.087 & 0.027 & 0.1673  \\
 	
 		\hline
 	CGN  	& Multi-Obj & 0.221 & 0.155 & 0.441 & 0.542 & 0.285 & 0.514 & 0.784 & 0.345 & 0.544  \\
 		\hline
 		
 	netNameS	& Single-Obj & 0.108 & 0.055 & 0.287 & 0.306 & 0.187 & 0.518 & 0.496 & 0.338 & 0.624  \\
 		\hline
  \end{tabular}
  \label{tab:visMulti}
  \end{threeparttable}
  \vspace*{-0.0 in}
\end{table*}

==> tables/tabVisSingle.tex <==
%\begin{table}[t!]
%  \centering
%  \setlength\tabcolsep{2.5 pt} 
%  \renewcommand{\arraystretch}{1.1}
%     \caption{Single-object Dataset Evaluation}
%  \begin{threeparttable}
%  \begin{tabular}{|c| c | c | c | c | c | c | c | c | c | c|c|}
%  		\hline
%	\multirow{2}{*}{Methods} &
%	\multirow{2}{*}{Modality} &
%    \multicolumn{3}{c|}{$1\text{cm}+20^\circ$} &
%    \multicolumn{3}{c|}{$2\text{cm}+30^\circ$} & 
%    \multicolumn{3}{c|}{$3\text{cm}+45^\circ$} & 
%    \multirow{2}{*}{FPS} \\ 
% 		\cline{3-11}
% 	{} & {} & GSR & GCR & OSR & GSR & GCR & OSR & GSR & GCR & OSR & {} \\
% 	\hline
% 	
% 	PnGPD 				& \multirow{2}{*}{\makecell{Point \\ Cloud}} & 0.004 &	0.001 & 0.015 &	0.015 & 0.009 & 0.036 & 0.205 & 0.048 & 0.160  & 0.008 \\ 
% 		
% 	6D-GN  	& {} & 0.039 & 0.068 & 0.354 & 0.165 & 0.396 & 0.791 & 0.359 & \textbf{0.739} & 0.977 & 0.240 \\
% 	CGN  	& {} & 0.299 & 0.249 & 0.770 & 0.601 & 0.320 & 0.817 & 0.816 & 0.365 & 0.842 & 2.108 \\
% 	
% 		\hline
% 		
% 	\netNameS	& RGB-D & \textbf{0.544} & \textbf{0.429} & \textbf{0.97} & \textbf{0.785} & \textbf{0.633} & \textbf{0.996} & \textbf{0.869} & 0.732 & \textbf{0.999} & \textbf{9.295} \\
% 		\hline
%  \end{tabular}
%  \label{tab:visSingle}
%  \end{threeparttable}
%  \vspace*{-0.0 in}
%\end{table}

\begin{table}[t!]
  \centering
  \setlength\tabcolsep{2.5 pt} 
  \renewcommand{\arraystretch}{1.1}
     \caption{Single-object Dataset Evaluation}
  \begin{threeparttable}
  \begin{tabular}{|c| c | c | c | c | c | c | c | c | c | c|c|}
  		\hline
	\multirow{2}{*}{Methods} &
	\multirow{2}{*}{Modality} &
    \multicolumn{3}{c|}{$1\text{cm}+20^\circ$} &
    \multicolumn{3}{c|}{$2\text{cm}+30^\circ$} & 
    \multicolumn{3}{c|}{$3\text{cm}+45^\circ$} & 
    \multirow{2}{*}{FPS} \\ 
 		\cline{3-11}
 	{} & {} & \multicolumn{3}{c|}{GSR/GCR/OSR} & \multicolumn{3}{c|}{GSR/GCR/OSR} & \multicolumn{3}{c|}{GSR/GCR/OSR} & {} \\
 	\hline
 	
 	PnGPD 				& \multirow{2}{*}{\makecell{Point \\ Cloud}} & 
 	\multicolumn{3}{c|}{0.004 / 0.001 / 0.015} &
 	\multicolumn{3}{c|}{0.015 / 0.009 / 0.036} &
 	\multicolumn{3}{c|}{0.205 / 0.048 / 0.160} & 0.008 \\ 
 	\cline{3-11}
 		
 	6D-GN  	& {} & 0.039 & 0.068 & 0.354 & 0.165 & 0.396 & 0.791 & 0.359 & \textbf{0.739} & 0.977 & 0.240 \\
 	CGN  	& {} & 0.299 & 0.249 & 0.770 & 0.601 & 0.320 & 0.817 & 0.816 & 0.365 & 0.842 & 2.108 \\
 	
 		\hline
 		
 	\netNameS	& RGB-D & \textbf{0.544} & \textbf{0.429} & \textbf{0.97} & \textbf{0.785} & \textbf{0.633} & \textbf{0.996} & \textbf{0.869} & 0.732 & \textbf{0.999} & \textbf{9.295} \\
 		\hline
  \end{tabular}
  \label{tab:visSingle}
  \end{threeparttable}
  \vspace*{-0.0 in}
\end{table}
